Call Graph Soundness in Android Static Analysis

Static analysis is sound in theory, but an implementation may unsoundly fail to analyze all of a program's code. Any such omission is a serious threat to the validity of the tool's output. Our work is the first to measure the prevalence of these omissions. Previously, researchers and analysts did not know what is missed by static analysis, what sort of code is missed, or the reasons behind these omissions. To address this gap, we ran 13 static analysis tools and a dynamic analysis on 1000 Android apps. Any method in the dynamic analysis but not in a static analysis is an unsoundness. Our findings include the following. (1) Apps built around external frameworks challenge static analyzers. On average, the 13 static analysis tools failed to capture 61% of the dynamically-executed methods. (2) A high level of precision in call graph construction is a synonym for a high level of unsoundness; (3) No existing approach significantly improves static analysis soundness. This includes those specifically tailored for a given mechanism, such as DroidRA to address reflection. It also includes systematic approaches, such as EdgeMiner, capturing all callbacks in the Android framework systematically. (4) Modeling entry point methods challenges call graph construction which jeopardizes soundness.

==> sections/rq5.tex <==
\subsubsection{Qualitative analysis}

In our qualitative analysis, we first compile all non-library methods missed by every static analyzer across all call graph construction algorithms into a new set: $\bigcup (DM^{\neg l} \setminus SM^{\neg l}_{cg})$. 
We then arrange these methods by frequency of occurrence. 
The findings will be presented in two stages: 
\dcircle{1} an examination of all methods; and
\dcircle{2} a focus on methods likely to be implicit mechanisms (the intent is two-fold: \dcircle{1} implicit mechanisms are likely to be missed by static analyzers since do call to implicit methods appear in apps' code; and \dcircle{2} discovering previously unknown implicit mechanisms that analysts and researchers overlook).



\noindent
\textbf{All Methods.}
Table~\ref{tab:missed_methods} shows the top 10 most frequently missed methods by all static analyzers in this study. 
Two key observations can be made: 
\dcircle{1} the top five methods all belong to the com.ryanheise package, which, after further investigation, appears to be a Flutter plugin\footnote{https://github.com/ryanheise/audio\_service}. 
Flutter is a framework for building apps.
\dcircle{2} the following five most frequently missed methods seem to have obfuscated names, preventing us from identifying their origin (are they framework or plugin methods that have been obfuscated?).
In addition, eight out of these 10 methods are class constructors (In Java, <init> refers to a constructor method, and <clinit> signifies a class initialization method, also known as a static initializer). 
The remaining two methods, onCreate()--a lifecycle method of the AudioService class that extends the MediaBrowserServiceCompat class--and size(), were called during run time but not modeled statically. 
This is unusual, given that static analyzers like FlowDroid are expected to handle lifecycle methods and other standard methods such as constructors.
The Flutter plugin may complicate static analysis as frameworks are inherently \emph{hard} to analyze. 
Table~\ref{tab:missed_methods} clearly shows that using frameworks like Flutter presents a significant obstacle to the precise static modeling of Android apps.

For a more precise view, we also examined the top 10 methods with non-obfuscated names. 
Table~\ref{tab:missed_methods_non_obfuscated} displays these findings. 
The top five remain the same as in Table~\ref{tab:missed_methods}. 
However, the remaining five methods reveal something interesting.
One method comes from the previously discussed Flutter plugin, and the other four belong to the same package: vn.hunghd.flutterdownloader, another Flutter plugin\footnote{https://github.com/fluttercommunity/flutter\_downloader}. 
This underscores the challenges that frameworks pose for static analyzers.

\begin{table}
    \centering
    \caption{Top 10 most missed methods by static analyzers without obfuscated methods.}
    \label{tab:missed_methods}
    \begin{adjustbox}{width=.8\columnwidth,center}
    \begin{tabular}{|c|c|}
        \hline
        Occurrence & Method \\
        \hline
        2190 & com.ryanheise.audioservice.AudioService.<init>() \\
        2190 & com.ryanheise.audioservice.AudioService.<clinit>() \\
        2165 & com.ryanheise.audioservice.AudioService\$d.<init>(AudioService) \\
        2159 & com.ryanheise.audioservice.AudioService.onCreate() \\
        2158 & com.ryanheise.audioservice.AudioService\$a.<init>(AudioService,int) \\
        2039 & l.b.<init>() \\
        1997 & k.a.<init>() \\
        1949 & k.b.<init>() \\
        1928 & r.g.<init>() \\
        1924 & l.b:.size() \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

\begin{table}
    \centering
    \caption{Top 10 most missed methods by static analyzers without obfuscated methods.}
    \label{tab:missed_methods_non_obfuscated}
    \begin{adjustbox}{width=.8\columnwidth,center}
    \begin{tabular}{|c|c|}
        \hline
        Occurrence & Method \\
        \hline
        2190 & com.ryanheise.audioservice.AudioService.<init>() \\
        2190 & com.ryanheise.audioservice.AudioService.<clinit>() \\
        2165 & com.ryanheise.audioservice.AudioService\$d.<init>(AudioService) \\
        2159 & com.ryanheise.audioservice.AudioService.onCreate() \\
        2158 & com.ryanheise.audioservice.AudioService\$a.<init>(AudioService,int) \\
        1781 & vn.hunghd.flutterdownloader.FlutterDownloaderInitializer.a(Context) \\
        1781 & vn.hunghd.flutterdownloader.FlutterDownloaderInitializer.<init>() \\
        1781 & vn.hunghd.flutterdownloader.FlutterDownloaderInitializer.onCreate() \\
        1771 & <com.ryanheise.audioservice.a.B(Context)> \\
        1770 & vn.hunghd.flutterdownloader.FlutterDownloaderInitializer\$a.<init>() \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}


\noindent
\textbf{Implicit Mechanisms.}
Identifying methods that are called implicitly, i.e., methods that are not directly called within the app but instead by an external framework like Flutter or the Android framework itself, is a non-trivial task~\cite{cao2015edgeminer,columbus,10.1109/ICSE43902.2021.00126,10.1145/2931037.2931044}. 
To improve our chances of discovering potential implicit mechanisms, we have employed a heuristic-based approach.
Our strategy involves selecting methods that were missed by the static analyzers and that also have names beginning with specific patterns: "on", "do", "handle", "dispatch", "perform", or "shouldOverride". 
The rationale behind choosing these patterns is because they are commonly found in known implicit mechanisms.
For example, in Android apps, methods that begin with "on" are typically associated with event listeners or lifecycle callbacks, like onCreate(), onStart(), or onClick(). 
Similarly, methods starting with "handle" or "perform" are often related to managing specific actions or events (e.g., handleMessage(message) or performClick()).
The "do" prefix is also used for methods that perform a specific action in response to an event, for example, doClick(View).
Methods with the "dispatch" prefix are usually associated with the propagation of events, like dispatchTouchEvent(MotionEvent).
A method named `shouldOverride` is likely to be used for customizing the behavior of an inherited method from an external framework (e.g., shouldOverrideUrlLoading(WebView, String)).

\begin{table}
    \centering
    \caption{Top 10 most missed methods by static analyzers likely to be implicit mechanisms}
    \label{tab:missed_methods_implicit}
    \begin{adjustbox}{width=.8\columnwidth,center}
    \begin{tabular}{|c|c|}
        \hline
        Occurrence & Method \\
        \hline
        2159 & com.ryanheise.audioservice.AudioService.onCreate() \\
        1781 & vn.hunghd.flutterdownloader.FlutterDownloaderInitializer.onCreate() \\
        1380 & okhttp3.OkHttpClient.dispatcher() \\
        1194 & r0.b\$a.onOpen(android.database.sqlite.SQLiteDatabase) \\
        1176 & r0.b\$a.onConfigure(android.database.sqlite.SQLiteDatabase) \\
        1040 & com.ironsource.lifecycle.b.onStop() \\
        1032 & com.ironsource.lifecycle.d.onActivityStopped(android.app.Activity) \\
        996 & com.ironsource.lifecycle.b.onPause() \\
        995 & com.ironsource.lifecycle.d.onActivityPaused(android.app.Activity) \\
        968 & okhttp3.CacheControl.onlyIfCached() \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

The results of this study are visible in Table~\ref{tab:missed_methods_implicit}.
Our analysis first reveals that the prefix "on" is the most prevalent among the top 10 missed methods that match our predefined prefix patterns.
Only one method employs the prefix "dispatch."
We note the presence of numerous --probable-- lifecycle methods, such as onCreate(), onStop(), onPause(), onActivityStopped(), and onActivityPaused(), that have been missed by static analyzers.

After further investigation, the onOpen() and onConfigure() methods are implicit mechanisms that are triggered by external frameworks, linked to database event handling.
As we analyzer deeper the top 100 missed methods, we observe that 78 methods use the "on" prefix, 5 the "do" prefix, the "handle" prefix is seen in 15 cases, and the "dispatch" prefix in 2 cases, while none use the "perform" or "shouldOverride" prefixes.
These findings imply that a considerable number of event listeners and lifecycle methods are overlooked by current static analysis tools. 

To gain a more in-depth understanding of the methods likely acting as implicit mechanisms, we extracted the names of all methods from our set of missed methods.
We found a total of \num{1016} unique method names for a total of \num{16521} methods.
After ranking these unique methods based on their occurrence, we retained the top 20. 
These findings are summarized in Figure~\ref{fig:most_methods_uniq}.

A key observation from these results is that a majority of the missed methods correlate strongly with lifecycle events (e.g., onActivityStarted()), user interface interactions (e.g., onClick()), configuration events (e.g., onConfigure()), and key event dispatches (e.g., dispatchKeyEvent()).
This suggests that many of these methods are invoked indirectly by external frameworks, often as a response to user actions or system events.

The lists of methods missed are available in our repository.

These findings align with previous studies~\cite{10.1145/2666356.2594299,10.1145/3510003.3512766,BarrosJMVDdAE2015,10.1145/2931037.2931044,10.5555/2818754.2818791,10.1109/ICSE43902.2021.00126,gordon2015information,reunify}, highlighting that implicit mechanisms hinder the construction of static models of Android apps.
When analyzing the total number of all method occurrences, a total of \num{9658051} instances were observed.
In the case of the implicit mechanisms discussed in this section, \num{220406} instances were observed, accounting for a mere 2.3\% of the total count.
This indicates that while implicit mechanisms contribute to hindering precise static model of Android apps, they are not the sole source of these difficulties.

Furthermore, if we observe, in Figures~\ref{fig:avg_successor} and~\ref{fig:avg_successor_implicit} , the distribution of the average of the number of methods called (i.e., all successors in the optimal call graph) dynamically, per app (computed from the data extracted from apps' execution thanks to our instrumentation of methods' relationships, see Listing~\ref{code:instrumentation}), we can see that if a method is missed by a static analyzer, this is in fact hundreds of methods that will not be modeled, and not analyzed.

\begin{figure}
  \centering
  \begin{subfigure}{0.45\textwidth}
    \begin{adjustbox}{width=.8\columnwidth,center}
        \includegraphics[width=\linewidth]{static_analysis/plots/distribution_average_number_of_methods_executer_by_a_method.pdf}
    \end{adjustbox}
    \caption{Distribution of the average number of successors of methods called at execution time}
    \label{fig:avg_successor}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \begin{adjustbox}{width=.8\columnwidth,center}
        \includegraphics[width=\linewidth]{static_analysis/plots/distribution_average_number_of_methods_executer_by_a_method_implicit.pdf}
    \end{adjustbox}
    \caption{Distribution of the average number of successors of implicit methods called at execution time}
    \label{fig:avg_successor_implicit}
  \end{subfigure}
  \caption{Distributions of the average number of successors of methods called during our dynamic analysis}
  \label{fig:avg_successor_both}
\end{figure}



\begin{figure}
  \centering
    \includegraphics[width=.97\columnwidth]{plots/occurrences_by_method.pdf}
  \caption{Top 20 most unique missed method' names by static analyzers likely to be implicit mechanisms}
  \label{fig:most_methods_uniq}
\end{figure}

\highlight{
\textbf{RQ6 answer:}
Our study reveals that implicit mechanisms pose a significant challenge in creating sound static models of Android apps.
Although they account for only 2.3\% of methods missed by existing static analyzers, they in fact trigger many methods not modeled statically.
Moreover, it highlights a deeper problem with current static analysis tools, which frequently overlook even non-implicit methods like basic class methods and constructors, pointing towards the need for more robust approaches that effectively encompass these methods.
}

==> sections/table-all-apps.tex <==

\begin{table}
    \centering
    \caption{Methods in static call graphs, for all apps successfully analyzed by each tool independently.  (CG = call graph, M. = Methods,
     Avg. = Average). The denominator for the \% columns is the number of methods in apps.}
    \begin{adjustbox}{width=.9\columnwidth,center}
        \begin{tabular}{|>{\color{blue}}c|>{\color{blue}}c||>{\color{blue}}c|>{\color{blue}}c|>{\color{blue}}c||>{\color{blue}}c|>{\color{blue}}c|>{\color{blue}}c|}
            \hline
            &  &
            \multicolumn{3}{>{\color{blue}}c||}{\textbf{With libraries}} & 
            \multicolumn{3}{>{\color{blue}}c|}{\textbf{Without libraries}} \\ \cline{3-8}
            &  &
                \multicolumn{1}{>{\color{blue}}c|}{\textbf{Avg.}} &
                \multicolumn{1}{>{\color{blue}}c|}{\textbf{\% M.}} & 
                \multicolumn{1}{>{\color{blue}}c||}{\textbf{Avg.}} &
                \multicolumn{1}{>{\color{blue}}c|}{\textbf{Avg.}} &
                \multicolumn{1}{>{\color{blue}}c|}{\textbf{\% M.}} & 
                \multicolumn{1}{>{\color{blue}}c|}{\textbf{Avg.}}
                \\  
            & & \textbf{$|SM|$}  &  \textbf{in CG} & \textbf{$|SE|$}
            & \textbf{$|SM^{\neg l}|$}  &   \textbf{in CG} &\textbf{$|SE^{\neg l}|$}  \\ \hline
                    \multirow{4}{*}{FlowDroid} & CHA
                    & \num{129048}
					& \num{52}\%
					& \num{1872283}
					& \num{28507}
					& \num{71}\%
					& \num{430259}
                     \\ \cline{2-2} \cline{3-8}
                     & RTA
                    & \num{83055}
					& \num{32}\%
					& \num{500280}
					& \num{12609}
					& \num{56}\%
					& \num{97120}
                     \\ \cline{2-2} \cline{3-8}
                     & VTA
                    & \num{104506}
					& \num{28}\%
					& \num{369205}
					& \num{23752}
					& \num{48}\%
					& \num{105922}
                     \\ \cline{2-2} \cline{3-8}
                     & SPARK
                    & \num{106112}
					& \num{7}\%
					& \num{38124}
					& \num{18368}
					& \num{13}\%
					& \num{13234}
                     \\ \hline \hline
                    \multirow{4}{*}{IccTA} & CHA
                    & \num{128267}
					& \num{52}\%
					& \num{1863207}
					& \num{28432}
					& \num{71}\%
					& \num{437583}
                     \\ \cline{2-2} \cline{3-8}
                     & RTA
                    & \num{82762}
					& \num{32}\%
					& \num{496354}
					& \num{12641}
					& \num{56}\%
					& \num{99125}
                     \\ \cline{2-2} \cline{3-8}
                     & VTA
                    & \num{104983}
					& \num{28}\%
					& \num{376083}
					& \num{24008}
					& \num{48}\%
					& \num{106710}
                     \\ \cline{2-2} \cline{3-8}
                     & SPARK
                    & \num{106880}
					& \num{7}\%
					& \num{39690}
					& \num{19499}
					& \num{13}\%
					& \num{15085}
                     \\ \hline \hline
                    \multirow{4}{*}{RAICC} & CHA
                    & \num{131052}
					& \num{51}\%
					& \num{1911574}
					& \num{27111}
					& \num{70}\%
					& \num{417491}
                     \\ \cline{2-2} \cline{3-8}
                     & RTA
                    & \num{83379}
					& \num{32}\%
					& \num{507312}
					& \num{12575}
					& \num{56}\%
					& \num{96237}
                     \\ \cline{2-2} \cline{3-8}
                     & VTA
                    & \num{104807}
					& \num{28}\%
					& \num{376629}
					& \num{24410}
					& \num{48}\%
					& \num{106190}
                     \\ \cline{2-2} \cline{3-8}
                     & SPARK
                    & \num{114015}
					& \num{8}\%
					& \num{73514}
					& \num{26537}
					& \num{15}\%
					& \num{44087}
                     \\ \hline \hline
                    \multirow{4}{*}{DroidRA} & CHA
                    & \num{131012}
					& \num{51}\%
					& \num{1879714}
					& \num{27109}
					& \num{70}\%
					& \num{391642}
                     \\ \cline{2-2} \cline{3-8}
                     & RTA
                    & \num{83262}
					& \num{32}\%
					& \num{494222}
					& \num{12544}
					& \num{56}\%
					& \num{94565}
                     \\ \cline{2-2} \cline{3-8}
                     & VTA
                    & \num{105666}
					& \num{28}\%
					& \num{366555}
					& \num{24426}
					& \num{47}\%
					& \num{101419}
                     \\ \cline{2-2} \cline{3-8}
                     & SPARK
                    & \num{115554}
					& \num{8}\%
					& \num{52313}
					& \num{25919}
					& \num{15}\%
					& \num{21957}
                     \\ \hline \hline
                    \multirow{1}{*}{NatiDroid} & CHA
                    & \num{75605}
					& \num{81}\%
					& \num{718644}
					& \num{11454}
					& \num{87}\%
					& \num{130550}
                     \\ \hline \hline
                    \multirow{1}{*}{MaMaDroid} & SPARK
                    & \num{70370}
					& \num{5}\%
					& \num{13807}
					& \num{9464}
					& \num{10}\%
					& \num{3015}
                     \\ \hline \hline
                    \multirow{1}{*}{BackDroid} & SPARK
                    & \num{70370}
					& \num{5}\%
					& \num{13816}
					& \num{9464}
					& \num{10}\%
					& \num{3015}
                     \\ \hline \hline
                    \multirow{1}{*}{SootFX} & SPARK
                    & \num{75510}
					& \num{0}\%
					& \num{124}
					& \num{11724}
					& \num{0}\%
					& \num{5}
                     \\ \hline \hline
                    \multirow{1}{*}{ACID} & SPARK
                    & \num{75529}
					& \num{7}\%
					& \num{77448}
					& \num{11717}
					& \num{26}\%
					& \num{8775}
                     \\ \hline \hline
                    \multirow{1}{*}{Gator} & CHA
                    & \num{118979}
					& \num{75}\%
					& \num{2293822}
					& \num{31605}
					& \num{90}\%
					& \num{715026}
                     \\ \hline \hline
                    \multirow{1}{*}{Jicer} & SPARK
                    & \num{111878}
					& \num{8}\%
					& \num{48816}
					& \num{23913}
					& \num{16}\%
					& \num{20842}
                     \\ \hline \hline
                    \multirow{1}{*}{ArpDroid} & SPARK
                    & \num{70370}
					& \num{5}\%
					& \num{13803}
					& \num{9464}
					& \num{10}\%
					& \num{3015}
                     \\ \hline \hline
                    \multirow{1}{*}{Difuzer} & CHA
                    & \num{71092}
					& \num{35}\%
					& \num{386057}
					& \num{6689}
					& \num{55}\%
					& \num{44848}
                     \\ \hline
        \end{tabular}
    \end{adjustbox}
    \label{table:results_statistic_all_apps}
\end{table}
